Reliable Detection of Doppelg\"angers based on Deep Face Representations

Doppelg\"angers (or lookalikes) usually yield an increased probability of false matches in a facial recognition system, as opposed to random face image pairs selected for non-mated comparison trials. In this work, we assess the impact of doppelg\"angers on the HDA Doppelg\"anger and Disguised Faces in The Wild databases using a state-of-the-art face recognition system. It is found that doppelg\"anger image pairs yield very high similarity scores resulting in a significant increase of false match rates. Further, we propose a doppelg\"anger detection method which distinguishes doppelg\"angers from mated comparison trials by analysing differences in deep representations obtained from face image pairs. The proposed detection system employs a machine learning-based classifier, which is trained with generated doppelg\"anger image pairs utilising face morphing techniques. Experimental evaluations conducted on the HDA Doppelg\"anger and Look-Alike Face databases reveal a detection equal error rate of approximately 2.7% for the task of separating mated authentication attempts from doppelg\"angers.

==> tab/detection_rates.tex <==
\begin{tabular}{lrrr}
\toprule
\textbf{Morphing Algorithm} & \textbf{D-EER} & \textbf{BPCER10} & \textbf{BPCER20} \\
\midrule
UBO & 2.57\% & 0.03\% & 0.45\% \\
FaceFusion & 2.79\% & 0.06\% & 0.48\% \\
%UBO+FaceFusion & 2.79\% & 0.06\% & 0.42\% \\
\bottomrule
\end{tabular}



==> tab/error_rates_doppelganger.tex <==
\begin{tabular}{llrr}
\toprule
\multirow{2}{*}{\textbf{Database}} & \multicolumn{3}{c}{\textbf{IAPMR at FMR of}} \\
\cmidrule{2-4}
& 1.00\% & 0.10\% & 0.01\% \\
\midrule
HDA-DG & 52.44\% & 29.82\% & 17.22\% \\
DFW & 39.70\% & 17.12\% & 6.85\% \\
\bottomrule
\end{tabular}

